An Overflow/Underflow-Free Fixed-Point Bit-Width Optimization Method for OS-ELM Digital Circuit

Currently there has been increasing demand for real-time training on resource-limited IoT devices such as smart sensors, which realizes standalone online adaptation for streaming data without data transfers to remote servers. OS-ELM (Online Sequential Extreme Learning Machine) has been one of promising neural-network-based online algorithms for on-chip learning because it can perform online training at low computational cost and is easy to implement as a digital circuit. Existing OS-ELM digital circuits employ fixed-point data format and the bit-widths are often manually tuned, however, this may cause overflow or underflow which can lead to unexpected behavior of the circuit. For on-chip learning systems, an overflow/underflow-free design has a great impact since online training is continuously performed and the intervals of intermediate variables will dynamically change as time goes by. In this paper, we propose an overflow/underflow-free bit-width optimization method for fixed-point digital circuits of OS-ELM. Experimental results show that our method realizes overflow/underflow-free OS-ELM digital circuits with 1.0x - 1.5x more area cost compared to the baseline simulation method where overflow or underflow can happen.

==> abst.tex <==

% abst.tex

\begin{summary}
Currently there has been increasing demand for real-time training on resource-limited IoT devices such as smart sensors,
which realizes standalone online adaptation for streaming data without data transfers to remote servers.
OS-ELM (Online Sequential Extreme Learning Machine) has been one of promising neural-network-based online algorithms for on-chip learning
because it can perform online training at low computational cost and is easy to implement as a digital circuit.
Existing OS-ELM digital circuits employ fixed-point data format and the bit-widths are often manually tuned, however, this may cause overflow or underflow
which can lead to unexpected behavior of the circuit.
For on-chip learning systems, an overflow/underflow-free design has a great impact since
online training is continuously performed and the intervals of intermediate variables will dynamically change as time goes by.
In this paper, we propose an overflow/underflow-free bit-width optimization method for fixed-point digital circuits of OS-ELM.
Experimental results show that our method realizes overflow/underflow-free OS-ELM digital circuits
with 1.0x - 1.5x more area cost compared to the baseline simulation method
where overflow or underflow can happen.
\end{summary}


==> related.tex <==
\section{Related Work}\label{sec:related}
\subsection{Static Interval Analysis for Iterative Algorithms}
Existing general-use static interval analysis methods,
including AA, deal with iterative algorithms by expanding them into feed-forward computation graphs using loop unrolling\cite{ia, aa, smtwlo_kinsman, hrwlo_boland}.
There must be a termination condition for the target iterative algorithm to apply loop unrolling; otherwise it cannot be represented in a feed-forward computation graph
and interval analysis becomes infeasible.
OS-ELM's training algorithm has no termination condition
and existing methods alone cannot realize interval analysis for OS-ELM.

Kinsman \textit{et al}. proposed an SMT (satisfiability modulo theory) based
static interval analysis framework designed for iterative algorithms \cite{kinsman_2011}
and demonstrated that the method worked for famous iterative algorithms, newton-raphson method
and conjugate gradient method, however,
it still cannot handle algorithms that do not have
termination conditions like OS-ELM.
Several papers \cite{lopez_2007, sarbishei_2010, sarbishei_2012, lamini_2014, ohno_2019} proposed analytical interval analysis methods
for LTI (linear time invariant) circuits with feedback loops
which cannot be translated into feed-forward computation graphs,
but the methods are dedicated to LTI circuits and not for OS-ELM.
As far as we know this paper is the first work to realize a static interval analysis
for OS-ELM by leveraging a numerical property of OS-ELM we pointed out in Section \ref{sec:method.train_analysis.n}.

\subsection{Division on Static Interval Analysis}
Most of static interval analysis methods assume that all denominators within a target algorithm do not take zero \cite{ia, aa, hrwlo_boland},
or interval analysis becomes infeasible.
SMT-based methods proposed by Kinsman \textit{et al}. provide a mitigation solution to handle a denominator that can take zero 
by forcibly adding a numerical constraint that prevents it from taking zero (e.g. $y \ge 0.01$ for $z = \frac{x}{y}$),
however, the constraint $y \ge 0.01$ is inconsistent with the fact $0 \in y$,
which can lead to overestimation or underestimation in subsequent intervals.

We took the safest strategy; we analytically proved that the denominator $\gamma^{(5)}_i = 1 + \bm{h}_i\bm{P}_{i-1}\bm{h}_i^T$ of OS-ELM
does not take zero at any $i \ge 1$, and proposed a mathematical trick based on the proof to safely represent OS-ELM in AA.
Note that the contributions can apply to not only AA but also other static interval analysis methods.

